Robustness of Bayesian Neural Networks to Gradient-Based Attacks

Vulnerability to adversarial attacks is one of the principal hurdles to the adoption of deep learning in safety-critical applications. Despite significant efforts, both practical and theoretical, the problem remains open. In this paper, we analyse the geometry of adversarial attacks in the large-data, overparametrized limit for Bayesian Neural Networks (BNNs). We show that, in the limit, vulnerability to gradient-based attacks arises as a result of degeneracy in the data distribution, i.e., when the data lies on a lower-dimensional submanifold of the ambient space. As a direct consequence, we demonstrate that in the limit BNN posteriors are robust to gradient-based adversarial attacks. Experimental results on the MNIST and Fashion MNIST datasets with BNNs trained with Hamiltonian Monte Carlo and Variational Inference support this line of argument, showing that BNNs can display both high accuracy and robustness to gradient based adversarial attacks.

==> Sections/GradientBasedAttacks.tex <==
\section{Gradient Based Adversarial Attacks}

%\ap{I have commented out a bit the white/black box bit of this. It is not discussed anywhere else in the paper so it might be a bit confusing to introduce it here imo.}

%We generally distinguish between two types of attacks, depending on the knowledge of the attacker about the structure of the model. White-box attacks have full access to the weights, the number of layers, the architecture and the hyperparameters of the classifier. Black-box attacks, on the other hand, are only aware of the training architecture or the output of the model on training samples.

Gradient-based attacks are among the most employed techniques for fast testing of NNs in adversarial settings. 
The basic principle is to perform gradient ascent on the loss to identify candidate adversarial perturbations.
Briefly,
%The most known adversarial attacks follow under the first category and are related to the principle of the gradient descent.
in the adversarial setting, instead of minimizing the loss function $L$ w.r.t. the NN weights on a given set (as in the training phase), the objective of the gradient method becomes loss maximization w.r.t. the input coordinates, while predictions of the network are performed with fixed weights. In other words, the gradient descent on the weights of the network becomes a local gradient ascent on the network input.

Specifically, let $f(\mathbf{x},\mathbf{w})$ be a NN with input $\mathbf{x}$ and network parameters (weights) $\mathbf{w}$, and denote by $L(f)$ the associated loss function. Given an input point $\mathbf{x}^*$, and a strength (i.e.\ maximum perturbation magnitude) $\epsilon>0$ of the attack, the worst-case adversarial perturbation can be defined as the point around $\mathbf{x}^*$ that maximises the loss:
%
$$\tilde{\mathbf{x}} := \argmax_{ \tilde{\mathbf{x}}:||\tilde{\mathbf{x}}-\mathbf{x}^*||_p \leq \epsilon} L (f(\tilde{\mathbf{x}},\mathbf{w})).$$
%
If the the network prediction on $\tilde{\mathbf{x}}$ differs from the original prediction on $\mathbf{x}^*$, then $\tilde{\mathbf{x}}$ is called an adversarial example.
As $f(\mathbf{x},\mathbf{w})$ is non-linear, this poses a non-linear optimisation problem for which several approximate solution methods have been proposed \citep{biggio2018wild}.
While the results discussed in Section \ref{sec:theory} hold for any gradient-based methods, in the experiments reported in Section \ref{sec:empirical_results} we directly look at the Fast Gradient Sign Method (FGSM) \citep{goodfellow2014explaining} and the Projected Gradient Descent method (PGD)  \citep{pgdattack}. The former,
FGSM, works by approximating $\tilde{\mathbf{x}}$ by taking an  $\epsilon$-step in the direction of the sign of the gradient in $\mathbf{x}$. In the case of $l_\infty$ perturbations, that is:
%
%
%The first \citet{goodfellow2014explaining} and one of the most used attacks, due to its simplicity and efficiency, is the Fast Gradient Sign Method (FGSM). This method aims at controlling the $l_p$ norm of the adversarial perturbation by adding noise in the direction of the loss gradient. In the case of $l_\infty$ norm, the perturbation is simply
$$\tilde{\mathbf{x}} \simeq  \mathbf{x}^* + \epsilon \cdot \text{sgn} \big(\nabla_\mathbf{x} L(f(\mathbf{x}^*,\mathbf{w}))\big).$$
%
PGD is based on a iterative generalisation of FGSM \citep{pgdattack}. It starts from a random perturbation  in an  $l_p$-ball of radius $\epsilon$ around the input sample $x^*$, then performs a gradient step in the direction of the greatest loss, projecting the so obtained point in the $\epsilon$-$l_p$-ball centered in $x^*$, and iterates the gradient step to improve approximations $\tilde{x}_t$:
\iffalse
through a projection $\mathcal{P}$
$$
\bm{\eta} \longleftarrow \mathcal{P}(\bm{\eta}+\alpha \cdot \nabla_{\bm{\eta}} L(f(\mathbf{w},\mathbf{x}+\bm{\eta}),y)).
$$
\fi
%
$$
\tilde{\mathbf{x}}^{t+1} =
Proj_{||\mathbf{x}^*-\tilde{\mathbf{x}}^t||_p \leq \epsilon}
\Big( 
\tilde{\mathbf{x}}^t+\alpha \cdot \text{sgn}~\nabla_{\mathbf{x}} L(f(\tilde{\mathbf{x}}^t,\mathbf{w}))
\Big).
$$
%
%By iteratively applying these steps, PGD solves the loss maximization problem.
%
%These two attack methods are used in the experimental section \ref{sec:empirical_results} as an empirical support to Theorem \ref{thm:main_statement}.
We stress that also attacks that do not rely directly on the gradient of the network under consideration have been developed \citep{papernot2017practical, ilyas2018black, wicker2018feature}.% Further there are gradient-based attacks which exist in the literature which we are not covering here, but that we expect would show similar results \citep{moosavi2016deepfool}.
